Zero-Crossing Precoding With Maximum Distance to the Decision Threshold for Channels With 1-Bit Quantization and Oversampling

Low-resolution devices are promising for systems that demand low energy consumption and low complexity as required in IoT systems. In this study, we propose a novel waveform for bandlimited channels with 1-bit quantization and oversampling at the receivers. The proposed method implies that the information is conveyed within the time instances of zero-crossings which is then utilized in combination with a Gray-coding scheme. Unlike the existing method, the proposed method does not require optimization and transmission of a dynamic codebook. The proposed approach outperforms the state-of-the-art method in terms of bit error rate.

==> MU_MIMO.tex <==
\section{Multiuser MIMO}
\label{sec:mu_mimo}
\begin{figure}[h]
\begin{center}
\captionsetup{justification=centering}
\includegraphics[width=9cm]{figures/modeloMIMO.eps}
\caption{Multiuser MIMO system model}
\label{fig:system_mimomodel}       % Give a unique label
\vspace{-0.8em}
\end{center}
\end{figure}



In this section the SISO system is extended to the multiuser MIMO system,
as 
shown in
Fig.~\ref{fig:system_mimomodel},
with $N_{\text{u}}$ single antenna users and $N_{\text{t}}$ transmit antennas at the BS, by following the approach in \cite{LarsonB_2017}. 
The symbol sequences of each user are processed and mapped by the ZC precoding \eqref{eq:convex} for each user $k$. 
The maximum transmit energy is equally spread among the users, such that ${E_{\text{Tx}}}= \frac{1}{2} E_{0} / N_{\text{u}}$.
The considered $N_{\text{u}} \times N_{\text{t}} $ channel matrix is denoted as   $\tilde{\boldsymbol{H}} = {\tilde{\boldsymbol{G}}} \boldsymbol{D_{\text{H}}}^{\frac{1}{2}}$, where $\tilde{\boldsymbol{G}}$ is the $N_{\text{u}} \times N_{\text{t}}$ matrix of fast fading coefficients described by a Rayleigh probability density function and the matrix $\boldsymbol{D_{\text{H}}} = \text{diag} \left ({\boldsymbol{\zeta}}/{\left ( {d}/{r_{d}} \right )^{\nu}}\right )$ models the geometric attenuation and shadow fading,
%\begin{align}
%      \boldsymbol{D_{\text{H}}} = \text{diag} \left ({\boldsymbol{\zeta}}/{\left ( \frac{d}{r_{d}} \right )^{\nu}}\right )\text{,}
%\end{align}
where $\zeta$ is a log-normal random variable with standard deviation $\sigma_{\text{shadow}}$, $d$ corresponds to the distance between the transmitter and the receiver, $r_{d}$  is the cell radius and $\nu$ is the path loss exponent \cite{Larson_2013}.
Note that we describe an equivalent discrete time model where the order of spatial precoding and pulse shaping filter is exchanged in the sequel.
Assuming perfect channel state information the spatial zero-forcing (ZF) precoding scheme \cite{SpencerHaardt_2004} reads
\begin{equation}
\label{eq:zf}
     \tilde{\boldsymbol{P}'}_{\text{zf}} = \tilde{\boldsymbol{H}}^{\text{H}}\left ( \tilde{\boldsymbol{H}}\tilde{\boldsymbol{H}}^{\text{H}} \right )^{-1} \quad \textrm{and} \quad \tilde{\boldsymbol{P}}_{\text{zf}} = c_{zf}\tilde{\boldsymbol{P}'}_{\text{zf}} \textrm{.}
\end{equation}
Defining ${\boldsymbol{P}}_{w} = \left [ (\boldsymbol{W}'{\boldsymbol{p}}_{\text{x}_{1}})^{\text{T}};(\boldsymbol{W}'{\boldsymbol{p}}_{\text{x}_{2}})^{\text{T}}; \cdots ; (\boldsymbol{W}'{\boldsymbol{p}}_{\text{x}_{N_{\text{u}}}})^{\text{T}}\right ]$ as the matrix of transmit signals and considering that the energy constraint holds with equality, yields  ${\boldsymbol{R}} = \mathbb{E}\left \{ {\boldsymbol{P}}_{w}{\boldsymbol{P}}_{w}^{\text{T}} \right \}  = E_{\text{Tx}} \boldsymbol{I}_{N_\text{u}}$. 
Including the precoding operation the energy constraint is given by $\text{trace}\left (\tilde{\boldsymbol{P}'}_{\text{zf}}{\boldsymbol{R}} \tilde{\boldsymbol{P}'}_{\text{zf}}^{\text{H}} \right ) = \frac{E_{\text{0}}}{2}$. With this, the factor in \eqref{eq:zf} reads  
\begin{align*}
\label{eq:czf}
c_{zf}  =  \left ( {N_{\text{u}}}/{\text{trace}\left ( \tilde{\boldsymbol{P}'}_{\text{zf}}\tilde{\boldsymbol{P}'}_{\text{zf}}^{\text{H}} \right )}  \right ) ^{\frac{1}{2}}     = 
\left (
{N_{\text{u}}}/{\textrm{trace}
\left (
\left ( \tilde{\boldsymbol{H}}\tilde{\boldsymbol{H}}^{{\text{H}}} \right )^{-1}}
\right )
\right ) ^{\frac{1}{2}}
\text{.}
\end{align*}
For ZF precoding, $\tilde{\boldsymbol{H}}\tilde{\boldsymbol{P}}_{\text{zf}}$ becomes a diagonal matrix $\beta \, \boldsymbol{I}_{N_{\text{u}}} $ where $\beta$ refers to the real valued beamforming gain. 
With this, the  received signal after the quantization is expressed as
\begin{align}
{\boldsymbol{z}} =   Q_{1}\left ( {\boldsymbol{y}} \right ) = Q_{1} \left ( \beta \left ( \boldsymbol{I}_{N_{\text{u}}} \otimes \boldsymbol{G}_{\text{tot}}\boldsymbol{U} \right ) {\boldsymbol{p}}_{x} + \left ( \boldsymbol{I}_{N_{\text{u}}} \otimes \boldsymbol{G}_{\text{s}} \right ){\boldsymbol{n}}\right ) \text{,}
\end{align}
where ${\boldsymbol{p}}_{x}$ is a stacked precoded vector with size $N_{\text{q}}N_{\text{u}} \times 1$ and ${\boldsymbol{n}}$ is a stacked noise vector with size $3N_{\text{tot}}N_{\text{u}} \times 1$. 
Accordingly, ${\boldsymbol{z}}$ is a stacked vector including the received signals for the $N_{\text{u}}$ users, each using the detector as described for the SISO case.
%In the MU-MIMO case  ${\boldsymbol{\beta}}$ is the stacked beamforming gain vector with size $N_{\text{q}}N_{\text{u}} \times 1$.\\
%In the MU-MIMO case:
%
%\begin{equation}
%{\boldsymbol{\beta}} =  \textrm{diag} \left ( \tilde{\boldsymbol{H}}\tilde{\boldsymbol{P}}_{\text{zf}} \otimes \boldsymbol{I}_{N_{\text{q}}}   \right )
%\end{equation}

%${\boldsymbol{\beta}}$ is the stacked beamforming gain vector with size $N_{\text{q}}N_{\text{u}} \times 1$
%As the quantized signal ${\boldsymbol{z}}$ is also a stacked vector, it is necessary to reshape ${\boldsymbol{z}}$ to get the sequence of each user i.e. ${\boldsymbol{z}}_{k}$ to perform the detection process since it is carried out in the same way as in the SISO case.




